GENIE-ASI: Generative Instruction and Executable Code for Analog Subcircuit Identification

Analog subcircuit identification is a core task in analog design, essential for simulation, sizing, and layout. Traditional methods often require extensive human expertise, rule-based encoding, or large labeled datasets. To address these challenges, we propose GENIE-ASI, the first training-free, large language model (LLM)-based methodology for analog subcircuit identification. GENIE-ASI operates in two phases: it first uses in-context learning to derive natural language instructions from a few demonstration examples, then translates these into executable Python code to identify subcircuits in unseen SPICE netlists. In addition, to evaluate LLM-based approaches systematically, we introduce a new benchmark composed of operational amplifier netlists (op-amps) that cover a wide range of subcircuit variants. Experimental results on the proposed benchmark show that GENIE-ASI matches rule-based performance on simple structures (F1-score = 1.0), remains competitive on moderate abstractions (F1-score = 0.81), and shows potential even on complex subcircuits (F1-score = 0.31). These findings demonstrate that LLMs can serve as adaptable, general-purpose tools in analog design automation, opening new research directions for foundation model applications in analog design automation.

==> tables/main_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\caption{Comparison between GENIE-ASI (\textit{Instruction + Code Generation}) and other baseline approaches.}
\setlength\tabcolsep{2.9pt} % default value: 6pt
\begin{adjustbox}{scale=0.64, center}

\begin{tabular}{ll|cccccccccccccccccc|cccccccccccccccccc}
\hline
\multicolumn{2}{l|}{\multirow{2}{*}{\textbf{Approach}}} &
  \multicolumn{18}{c|}{\textbf{Two-stage Approaches}} &
  \multicolumn{18}{c}{\textbf{One-Stage Approaches}} \\ \cline{3-38} 
\multicolumn{2}{l|}{} &
  \multicolumn{9}{c|}{\textbf{Instruction + Code   Generation}} &
  \multicolumn{9}{c|}{\textbf{Instruction + Following}} &
  \multicolumn{9}{c|}{\textbf{Direct Prompting}} &
  \multicolumn{9}{c}{\textbf{Direct Code Generation}} \\ \hline
\multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Model}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Metrics}}} &
  \multicolumn{3}{c|}{\textbf{S}} &
  \multicolumn{3}{c|}{\textbf{M}} &
  \multicolumn{3}{c|}{\textbf{L}} &
  \multicolumn{3}{c|}{\textbf{S}} &
  \multicolumn{3}{c|}{\textbf{M}} &
  \multicolumn{3}{c|}{\textbf{L}} &
  \multicolumn{3}{c|}{\textbf{S}} &
  \multicolumn{3}{c|}{\textbf{M}} &
  \multicolumn{3}{c|}{\textbf{L}} &
  \multicolumn{3}{c|}{\textbf{S}} &
  \multicolumn{3}{c|}{\textbf{M}} &
  \multicolumn{3}{c}{\textbf{L}} \\ \cline{3-38} 
\multicolumn{1}{l|}{} &
  \multicolumn{1}{c|}{} &
  HL1 &
  HL2 &
  \multicolumn{1}{c|}{HL3} &
  HL1 &
  HL2 &
  \multicolumn{1}{c|}{HL3} &
  HL1 &
  HL2 &
  \multicolumn{1}{c|}{HL3} &
  HL1 &
  HL2 &
  \multicolumn{1}{c|}{HL3} &
  HL1 &
  HL2 &
  \multicolumn{1}{c|}{HL3} &
  HL1 &
  HL2 &
  HL3 &
  HL1 &
  HL2 &
  \multicolumn{1}{c|}{HL3} &
  HL1 &
  HL2 &
  \multicolumn{1}{c|}{HL3} &
  HL1 &
  HL2 &
  \multicolumn{1}{c|}{HL3} &
  HL1 &
  HL2 &
  \multicolumn{1}{c|}{HL3} &
  HL1 &
  HL2 &
  \multicolumn{1}{c|}{HL3} &
  HL1 &
  HL2 &
  HL3 \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{gpt-4.1}} &
  PR &
  1.00 &
  0.96 &
  \multicolumn{1}{c|}{0.25} &
  1.00 &
  1.00 &
  \multicolumn{1}{c|}{0.22} &
  1.00 &
  1.00 &
  \multicolumn{1}{c|}{0.17} &
  0.94 &
  0.69 &
  \multicolumn{1}{c|}{0.30} &
  0.95 &
  0.65 &
  \multicolumn{1}{c|}{0.25} &
  0.92 &
  0.75 &
  0.24 &
  0.87 &
  0.43 &
  \multicolumn{1}{c|}{0.21} &
  0.86 &
  0.45 &
  \multicolumn{1}{c|}{0.17} &
  0.77 &
  0.47 &
  \multicolumn{1}{c|}{0.12} &
  1.00 &
  0.81 &
  \multicolumn{1}{c|}{0.06} &
  1.00 &
  0.73 &
  \multicolumn{1}{c|}{0.06} &
  1.00 &
  0.69 &
  0.03 \\
\multicolumn{1}{l|}{} &
  RC &
  0.99 &
  0.74 &
  \multicolumn{1}{c|}{0.25} &
  0.93 &
  0.78 &
  \multicolumn{1}{c|}{0.22} &
  0.91 &
  0.77 &
  \multicolumn{1}{c|}{0.17} &
  1.00 &
  0.53 &
  \multicolumn{1}{c|}{0.26} &
  0.99 &
  0.48 &
  \multicolumn{1}{c|}{0.20} &
  0.98 &
  0.45 &
  0.16 &
  0.95 &
  0.39 &
  \multicolumn{1}{c|}{0.20} &
  0.93 &
  0.41 &
  \multicolumn{1}{c|}{0.17} &
  0.92 &
  0.39 &
  \multicolumn{1}{c|}{0.12} &
  0.95 &
  0.54 &
  \multicolumn{1}{c|}{0.06} &
  0.92 &
  0.51 &
  \multicolumn{1}{c|}{0.06} &
  0.87 &
  0.49 &
  0.03 \\
\multicolumn{1}{l|}{} &
  F1-score &
  0.99 &
  0.83 &
  \multicolumn{1}{c|}{0.25} &
  0.96 &
  0.87 &
  \multicolumn{1}{c|}{0.22} &
  0.95 &
  0.87 &
  \multicolumn{1}{c|}{0.17} &
  1.00 &
  0.59 &
  \multicolumn{1}{c|}{0.28} &
  0.97 &
  0.54 &
  \multicolumn{1}{c|}{0.22} &
  0.94 &
  0.54 &
  0.19 &
  0.90 &
  0.41 &
  \multicolumn{1}{c|}{0.20} &
  0.88 &
  0.42 &
  \multicolumn{1}{c|}{0.17} &
  0.82 &
  0.42 &
  \multicolumn{1}{c|}{0.12} &
  0.97 &
  0.64 &
  \multicolumn{1}{c|}{0.06} &
  0.96 &
  0.60 &
  \multicolumn{1}{c|}{0.06} &
  0.93 &
  0.57 &
  0.03 \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{grok-3-beta}} &
  PR &
  1.00 &
  0.99 &
  \multicolumn{1}{c|}{0.16} &
  1.00 &
  0.96 &
  \multicolumn{1}{c|}{0.11} &
  1.00 &
  0.97 &
  \multicolumn{1}{c|}{0.07} &
   &
  0.58 &
  \multicolumn{1}{c|}{} &
   &
  0.60 &
  \multicolumn{1}{c|}{} &
   &
   &
   &
  0.90 &
  0.64 &
  \multicolumn{1}{c|}{0.26} &
  0.86 &
  0.57 &
  \multicolumn{1}{c|}{0.15} &
  0.85 &
  0.40 &
  \multicolumn{1}{c|}{0.15} &
  1.00 &
  0.28 &
  \multicolumn{1}{c|}{0.14} &
  1.00 &
  0.27 &
  \multicolumn{1}{c|}{0.09} &
  1.00 &
  0.26 &
  0.06 \\
\multicolumn{1}{l|}{} &
  RC &
  1.00 &
  0.62 &
  \multicolumn{1}{c|}{0.16} &
  1.00 &
  0.60 &
  \multicolumn{1}{c|}{0.11} &
  1.00 &
  0.62 &
  \multicolumn{1}{c|}{0.07} &
   &
  0.54 &
  \multicolumn{1}{c|}{} &
   &
  0.56 &
  \multicolumn{1}{c|}{} &
   &
   &
   &
  0.98 &
  0.53 &
  \multicolumn{1}{c|}{0.27} &
  0.97 &
  0.49 &
  \multicolumn{1}{c|}{0.15} &
  0.92 &
  0.34 &
  \multicolumn{1}{c|}{0.15} &
  1.00 &
  0.21 &
  \multicolumn{1}{c|}{0.14} &
  1.00 &
  0.22 &
  \multicolumn{1}{c|}{0.09} &
  1.00 &
  0.22 &
  0.06 \\
\multicolumn{1}{l|}{} &
  F1-score &
  1.00 &
  0.75 &
  \multicolumn{1}{c|}{0.16} &
  1.00 &
  0.73 &
  \multicolumn{1}{c|}{0.11} &
  1.00 &
  0.76 &
  \multicolumn{1}{c|}{0.07} &
   &
  0.56 &
  \multicolumn{1}{c|}{} &
   &
  0.60 &
  \multicolumn{1}{c|}{} &
   &
   &
   &
  0.93 &
  0.58 &
  \multicolumn{1}{c|}{0.27} &
  0.89 &
  0.52 &
  \multicolumn{1}{c|}{0.15} &
  0.87 &
  0.36 &
  \multicolumn{1}{c|}{0.15} &
  1.00 &
  0.24 &
  \multicolumn{1}{c|}{0.14} &
  1.00 &
  0.24 &
  \multicolumn{1}{c|}{0.09} &
  1.00 &
  0.23 &
  0.06 \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{deepseek-r1}} &
  PR &
  1.00 &
  0.32 &
  \multicolumn{1}{c|}{0.14} &
  1.00 &
  0.30 &
  \multicolumn{1}{c|}{0.10} &
  1.00 &
  0.34 &
  \multicolumn{1}{c|}{0.07} &
   &
   &
  \multicolumn{1}{c|}{} &
   &
   &
  \multicolumn{1}{c|}{} &
   &
   &
   &
   &
   &
  \multicolumn{1}{c|}{} &
   &
   &
  \multicolumn{1}{c|}{} &
   &
   &
  \multicolumn{1}{c|}{} &
  1.00 &
  0.01 &
  \multicolumn{1}{c|}{0.10} &
  1.00 &
  0.04 &
  \multicolumn{1}{c|}{0.06} &
  1.00 &
  0.04 &
  0.03 \\
\multicolumn{1}{l|}{} &
  RC &
  1.00 &
  0.33 &
  \multicolumn{1}{c|}{0.13} &
  1.00 &
  0.34 &
  \multicolumn{1}{c|}{0.09} &
  1.00 &
  0.41 &
  \multicolumn{1}{c|}{0.07} &
   &
   &
  \multicolumn{1}{c|}{} &
   &
   &
  \multicolumn{1}{c|}{} &
   &
   &
   &
   &
   &
  \multicolumn{1}{c|}{} &
   &
   &
  \multicolumn{1}{c|}{} &
   &
   &
  \multicolumn{1}{c|}{} &
  0.98 &
  0.01 &
  \multicolumn{1}{c|}{0.10} &
  0.88 &
  0.03 &
  \multicolumn{1}{c|}{0.06} &
  0.82 &
  0.03 &
  0.03 \\
\multicolumn{1}{l|}{} &
  F1-score &
  1.00 &
  0.33 &
  \multicolumn{1}{c|}{0.13} &
  1.00 &
  0.32 &
  \multicolumn{1}{c|}{0.10} &
  1.00 &
  0.37 &
  \multicolumn{1}{c|}{0.07} &
   &
   &
  \multicolumn{1}{c|}{} &
   &
   &
  \multicolumn{1}{c|}{} &
   &
   &
   &
   &
   &
  \multicolumn{1}{c|}{} &
   &
   &
  \multicolumn{1}{c|}{} &
   &
   &
  \multicolumn{1}{c|}{} &
  0.99 &
  0.01 &
  \multicolumn{1}{c|}{0.10} &
  0.92 &
  0.03 &
  \multicolumn{1}{c|}{0.06} &
  0.89 &
  0.03 &
  0.03 \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{llama3.3:70b}} &
  PR &
  0.00 &
  0.62 &
  \multicolumn{1}{c|}{0.24} &
  0.00 &
  0.65 &
  \multicolumn{1}{c|}{0.20} &
  0.00 &
  0.71 &
  \multicolumn{1}{c|}{0.13} &
  0.79 &
  0.44 &
  \multicolumn{1}{c|}{0.333} &
  0.78 &
  0.38 &
  \multicolumn{1}{c|}{0.28} &
  0.76 &
  0.39 &
  0.25 &
  0.65 &
  0.48 &
  \multicolumn{1}{c|}{0.20} &
  0.70 &
  0.38 &
  \multicolumn{1}{c|}{0.14} &
  0.67 &
  0.41 &
  \multicolumn{1}{c|}{0.16} &
  1.00 &
  0.02 &
  \multicolumn{1}{c|}{0.20} &
  1.00 &
  0.00 &
  \multicolumn{1}{c|}{0.13} &
  1.00 &
  0.00 &
  0.07 \\
\multicolumn{1}{l|}{} &
  RC &
  0.00 &
  0.55 &
  \multicolumn{1}{c|}{0.22} &
  0.00 &
  0.55 &
  \multicolumn{1}{c|}{0.17} &
  0.00 &
  0.54 &
  \multicolumn{1}{c|}{0.10} &
  0.80 &
  0.42 &
  \multicolumn{1}{c|}{0.306} &
  0.77 &
  0.40 &
  \multicolumn{1}{c|}{0.25} &
  0.70 &
  0.40 &
  0.21 &
  0.67 &
  0.45 &
  \multicolumn{1}{c|}{0.20} &
  0.68 &
  0.40 &
  \multicolumn{1}{c|}{0.14} &
  0.61 &
  0.43 &
  \multicolumn{1}{c|}{0.15} &
  1.00 &
  0.00 &
  \multicolumn{1}{c|}{0.15} &
  1.00 &
  0.00 &
  \multicolumn{1}{c|}{0.11} &
  1.00 &
  0.00 &
  0.06 \\
\multicolumn{1}{l|}{} &
  F1-score &
  0.00 &
  0.58 &
  \multicolumn{1}{c|}{0.23} &
  0.00 &
  0.59 &
  \multicolumn{1}{c|}{0.18} &
  0.00 &
  0.61 &
  \multicolumn{1}{c|}{0.11} &
  0.79 &
  0.43 &
  \multicolumn{1}{c|}{0.318} &
  0.77 &
  0.00 &
  \multicolumn{1}{c|}{0.26} &
  0.72 &
  0.39 &
  0.23 &
  0.65 &
  0.46 &
  \multicolumn{1}{c|}{0.20} &
  0.68 &
  0.39 &
  \multicolumn{1}{c|}{0.14} &
  0.63 &
  0.42 &
  \multicolumn{1}{c|}{0.15} &
  1.00 &
  0.01 &
  \multicolumn{1}{c|}{0.18} &
  1.00 &
  0.00 &
  \multicolumn{1}{c|}{0.12} &
  1.00 &
  0.00 &
  0.07 \\ \hline
\end{tabular}


\end{adjustbox}
\label{table:main_result}
\end{table*}

==> tables/main_results_with_avg.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\caption{Comparison between GENIE-ASI (\textit{Instruction + Code Generation}) and other baseline approaches.}
\setlength\tabcolsep{2.9pt} % default value: 6pt
\begin{adjustbox}{scale=0.80, center}
\begin{tabular}{l|l|rr|rr}
\hline
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Metrics}} & \multicolumn{2}{c|}{\textbf{Two-phase Approaches}}                                             & \multicolumn{2}{c}{\textbf{One-phase Approaches}}                                \\ \cline{3-6} 
                                &                                   & \multicolumn{1}{r|}{\textit{Instruction + Code Generation}} & \textit{Instruction + Following} & \multicolumn{1}{r|}{\textit{Direct Prompting}} & \textit{Direct Code Generation} \\ \hline
                                & PR\_strict                        & \multicolumn{1}{r|}{\textbf{0.70}}                          & 0.64                             & \multicolumn{1}{r|}{0.55}                      & 0.64                            \\
                                & RC\_strict                        & \multicolumn{1}{r|}{\textbf{0.68}}                          & 0.64                             & \multicolumn{1}{r|}{0.57}                      & 0.64                            \\
                                & F1-score\_strict                  & \multicolumn{1}{r|}{\textbf{0.69}}                          & 0.63                             & \multicolumn{1}{r|}{0.55}                      & 0.64                            \\
gpt-4.1                         & PR                                & \multicolumn{1}{r|}{\textbf{0.79}}                          & 0.63                             & \multicolumn{1}{r|}{0.48}                      & 0.60                            \\
                                & RC                                & \multicolumn{1}{r|}{\textbf{0.66}}                          & 0.56                             & \multicolumn{1}{r|}{0.50}                      & 0.49                            \\
                                & F1-score                          & \multicolumn{1}{r|}{\textbf{0.71}}                          & 0.58                             & \multicolumn{1}{r|}{0.48}                      & 0.53                            \\ \hline
                                & PR\_strict                        & \multicolumn{1}{r|}{0.67}                                   & 0.67                             & \multicolumn{1}{r|}{0.60}                      & \textbf{0.71}                   \\
                                & RC\_strict                        & \multicolumn{1}{r|}{0.64}                                   & 0.68                             & \multicolumn{1}{r|}{0.62}                      & \textbf{0.73}                   \\
                                & F1-score\_strict                  & \multicolumn{1}{r|}{0.65}                                   & 0.67                             & \multicolumn{1}{r|}{0.60}                      & \textbf{0.71}                   \\
grok-3-beta                     & PR                                & \multicolumn{1}{r|}{\textbf{0.70}}                          & 0.56                             & \multicolumn{1}{r|}{0.53}                      & 0.46                            \\
                                & RC                                & \multicolumn{1}{r|}{\textbf{0.58}}                          & 0.58                             & \multicolumn{1}{r|}{0.53}                      & 0.44                            \\
                                & F1-score                          & \multicolumn{1}{r|}{\textbf{0.62}}                          & 0.56                             & \multicolumn{1}{r|}{0.52}                      & 0.44                            \\ \hline
                                & PR\_strict                        & \multicolumn{1}{r|}{\textbf{0.72}}                          & 0.67                             & \multicolumn{1}{r|}{0.71}                      & 0.52                            \\
                                & RC\_strict                        & \multicolumn{1}{r|}{\textbf{0.77}}                          & 0.67                             & \multicolumn{1}{r|}{0.71}                      & 0.52                            \\
                                & F1-score\_strict                  & \multicolumn{1}{r|}{\textbf{0.73}}                          & 0.66                             & \multicolumn{1}{r|}{0.70}                      & 0.52                            \\
deepseek-r1                     & PR                                & \multicolumn{1}{r|}{0.48}                                   & \textbf{0.70}                    & \multicolumn{1}{r|}{0.67}                      & 0.36                            \\
                                & RC                                & \multicolumn{1}{r|}{0.49}                                   & 0.60                             & \multicolumn{1}{r|}{\textbf{0.63}}             & 0.33                            \\
                                & F1-score                          & \multicolumn{1}{r|}{0.48}                                   & 0.63                             & \multicolumn{1}{r|}{\textbf{0.64}}             & 0.34                            \\ \hline
                                & PR\_strict                        & \multicolumn{1}{r|}{0.23}                                   & 0.50                             & \multicolumn{1}{r|}{0.44}                      & \textbf{0.47}                   \\
                                & RC\_strict                        & \multicolumn{1}{r|}{0.20}                                   & 0.54                             & \multicolumn{1}{r|}{\textbf{0.48}}             & 0.47                            \\
                                & F1-score\_strict                  & \multicolumn{1}{r|}{0.21}                                   & \textbf{0.50}                    & \multicolumn{1}{r|}{0.45}                      & 0.47                            \\
llama3.3:70b                    & PR                                & \multicolumn{1}{r|}{0.32}                                   & \textbf{0.49}                    & \multicolumn{1}{r|}{0.42}                      & 0.38                            \\
                                & RC                                & \multicolumn{1}{r|}{0.26}                                   & \textbf{0.47}                    & \multicolumn{1}{r|}{0.41}                      & 0.37                            \\
                                & F1-score                          & \multicolumn{1}{r|}{0.28}                                   & \textbf{0.43}                    & \multicolumn{1}{r|}{0.41}                      & 0.37                            \\ \hline
\end{tabular}
\end{adjustbox}
\label{table:main_result}
\end{table*}

==> tables/main_table_with_avg_horizontal.tex <==
\begin{table*}[]
\caption{Comparison between GENIE-ASI (\textit{Instruction + Code Generation}) and other LLM-based  approaches.}
\setlength\tabcolsep{3pt}
\begin{adjustbox}{scale=0.9, center}
\begin{tabular}{ll|cccccc}
\hline
\textbf{Model} & \textbf{Approach} & $\text{PR}_{strict}$ & $\text{RC}_{strict}$ & $\text{F1-score}_{strict}$ &  $\text{PR}$ & $\text{RC}$ & $\text{F1-score}$ \\
\hline
\multirow{4}{*}{gpt-4.1} 
  & Instruction + Code Generation & \textbf{0.70} & \textbf{0.68} & \textbf{0.69} & \textbf{0.79} & \textbf{0.66} & \textbf{0.71} \\
  & Instruction + Following       & 0.64 & 0.64 & 0.63 & 0.63 & 0.56 & 0.58 \\
  & Direct Prompting              & 0.55 & 0.57 & 0.55 & 0.48 & 0.50 & 0.48 \\
  & Direct Code Generation        & 0.64 & 0.64 & 0.64 & 0.60 & 0.49 & 0.53 \\
\hline
\multirow{4}{*}{grok-3-beta} 
  & Instruction + Code Generation & 0.67 & 0.64 & 0.65 & \textbf{0.70} & \textbf{0.58} & \textbf{0.62} \\
  & Instruction + Following       & 0.67 & 0.68 & 0.67 & 0.56 & 0.58 & 0.56 \\
  & Direct Prompting              & 0.60 & 0.62 & 0.60 & 0.53 & 0.53 & 0.52 \\
  & Direct Code Generation        & \textbf{0.71} & \textbf{0.73} & \textbf{0.71} & 0.46 & 0.44 & 0.44 \\
\hline
\multirow{4}{*}{deepseek-r1} 
  & Instruction + Code Generation & \textbf{0.72} & \textbf{0.77} & \textbf{0.73} & 0.48 & 0.49 & 0.48 \\
  & Instruction + Following       & 0.67 & 0.67 & 0.66 & \textbf{0.70} & 0.60 & 0.63 \\
  & Direct Prompting              & 0.71 & 0.71 & 0.70 & 0.67 & \textbf{0.63} & \textbf{0.64} \\
  & Direct Code Generation        & 0.52 & 0.52 & 0.52 & 0.36 & 0.33 & 0.34 \\
\hline
\multirow{4}{*}{llama3.3:70b} 
  & Instruction + Code Generation & 0.23 & 0.20 & 0.21 & 0.32 & 0.26 & 0.28 \\
  & Instruction + Following       & 0.50 & 0.54 & \textbf{0.50} & \textbf{0.49} & \textbf{0.47} & \textbf{0.43} \\
  & Direct Prompting              & 0.44 & \textbf{0.48} & 0.45 & 0.42 & 0.41 & 0.41 \\
  & Direct Code Generation        & \textbf{0.47} & 0.47 & 0.47 & 0.38 & 0.37 & 0.37 \\
\hline
\end{tabular}
\end{adjustbox}
\label{table:main_result}
\end{table*}


==> tables/table_compare_across_HL.tex <==

\begin{table*}[htbp]
\begin{minipage}{0.48\textwidth}
\caption{Comparison between GENIE-ASI (\textit{Instruction + Code Generation}) and other LLM-based  approaches.}
\centering
\setlength\tabcolsep{2pt}
\begin{adjustbox}{scale=0.77, center}
\begin{tabular}{ll|cccccc}
\hline
\textbf{Model} & \textbf{Approach} & $\text{PR}_{strict}$ & $\text{RC}_{strict}$ & $\text{F1-score}_{strict}$ &  $\text{PR}$ & $\text{RC}$ & $\text{F1-score}$ \\
\hline
\multirow{4}{*}{gpt-4.1} 
  & GENIE-ASI & \textbf{0.70} & \textbf{0.68} & \textbf{0.69} & \textbf{0.79} & \textbf{0.66} & \textbf{0.71} \\
  & Instruction + Following       & 0.64 & 0.64 & 0.63 & 0.63 & 0.56 & 0.58 \\
  & Direct Prompting              & 0.55 & 0.57 & 0.55 & 0.48 & 0.50 & 0.48 \\
  & Direct Code Generation        & 0.64 & 0.64 & 0.64 & 0.60 & 0.49 & 0.53 \\
\hline
\multirow{4}{*}{grok-3-beta} 
  & GENIE-ASI & 0.67 & 0.64 & 0.65 & \textbf{0.70} & \textbf{0.58} & \textbf{0.62} \\
  & Instruction + Following       & 0.67 & 0.68 & 0.67 & 0.56 & 0.58 & 0.56 \\
  & Direct Prompting              & 0.60 & 0.62 & 0.60 & 0.53 & 0.53 & 0.52 \\
  & Direct Code Generation        & \textbf{0.71} & \textbf{0.73} & \textbf{0.71} & 0.46 & 0.44 & 0.44 \\
\hline
\multirow{4}{*}{deepseek-r1} 
  & GENIE-ASI & \textbf{0.72} & \textbf{0.77} & \textbf{0.73} & 0.48 & 0.49 & 0.48 \\
  & Instruction + Following       & 0.67 & 0.67 & 0.66 & \textbf{0.70} & 0.60 & 0.63 \\
  & Direct Prompting              & 0.71 & 0.71 & 0.70 & 0.67 & \textbf{0.63} & \textbf{0.64} \\
  & Direct Code Generation        & 0.52 & 0.52 & 0.52 & 0.36 & 0.33 & 0.34 \\
\hline
\multirow{4}{*}{llama3.3:70b} 
  & GENIE-ASI & 0.23 & 0.20 & 0.21 & 0.32 & 0.26 & 0.28 \\
  & Instruction + Following       & 0.50 & 0.54 & \textbf{0.50} & \textbf{0.49} & \textbf{0.47} & \textbf{0.43} \\
  & Direct Prompting              & 0.44 & \textbf{0.48} & 0.45 & 0.42 & 0.41 & 0.41 \\
  & Direct Code Generation        & \textbf{0.47} & 0.47 & 0.47 & 0.38 & 0.37 & 0.37 \\
\hline
\end{tabular}

\end{adjustbox}

\label{table:main_result}
\end{minipage}
\hfill
\begin{minipage}{0.48\textwidth}
\caption{Model Performance Across Hierarchy Levels (HL1–HL3) Under GENIE-ASI and LLM-based Approaches}
\centering

\setlength\tabcolsep{2pt}
\begin{adjustbox}{scale=0.88, center}
\begin{tabular}{l|l|rrr|rrr|rrr|rrr}
\hline
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Metrics}} & \multicolumn{3}{c|}{\textbf{GENIE-ASI}}                  & \multicolumn{3}{c|}{\textbf{Inst+Following}}                          & \multicolumn{3}{c|}{\textbf{Direct Prompt}}                                  & \multicolumn{3}{c}{\textbf{Direct Code}}                         \\ \cline{3-14} 
                                &                                   & \multicolumn{1}{c}{HL1} & \multicolumn{1}{c}{HL2} & \multicolumn{1}{c|}{HL3} & \multicolumn{1}{c}{HL1} & \multicolumn{1}{c}{HL2} & \multicolumn{1}{c|}{HL3} & \multicolumn{1}{c}{HL1} & \multicolumn{1}{c}{HL2} & \multicolumn{1}{c|}{HL3} & \multicolumn{1}{c}{HL1} & \multicolumn{1}{c}{HL2} & \multicolumn{1}{c}{HL3} \\ \hline
\multirow{3}{*}{gpt-4.1}        & PR                                & \textbf{1.00}           & \textbf{0.99}           & \textbf{0.38}            & 0.94                    & 0.70                    & 0.26                     & 0.83                    & 0.45                    & 0.17                     & \textbf{1.00}           & 0.75                    & 0.05                    \\
                                & RC                                & \textbf{0.94}           & \textbf{0.77}           & \textbf{0.26}            & \textbf{0.99}           & 0.49                    & 0.21                     & 0.93                    & 0.40                    & 0.16                     & 0.91                    & 0.51                    & 0.05                    \\
                                & F1-score                          & \textbf{0.97}           & 0.86                    & 0.31                     & 0.97                    & 0.56                    & 0.23                     & 0.86                    & 0.42                    & 0.16                     & 0.95                    & 0.60                    & 0.05                    \\ \hline
\multirow{3}{*}{grok-3-beta}    & PR                                & \textbf{1.00}           & \textbf{0.97}           & 0.11                     & 0.87                    & 0.61                    & 0.21                     & 0.87                    & 0.54                    & \textbf{0.19}            & \textbf{1.00}           & 0.27                    & 0.10                    \\
                                & RC                                & \textbf{1.00}           & \textbf{0.61}           & 0.11                     & 0.98                    & 0.55                    & \textbf{0.21}            & 0.96                    & 0.46                    & 0.19                     & 1.00                    & 0.22                    & 0.10                    \\
                                & F1-score                          & \textbf{1.00}           & 0.74                    & 0.11                     & 0.91                    & 0.57                    & 0.21                     & 0.90                    & 0.49                    & 0.19                     & 1.00                    & 0.24                    & 0.10                    \\ \hline
\multirow{3}{*}{deepseek-r1}    & PR                                & \textbf{1.00}           & 0.32                    & 0.10                     & \textbf{1.00}           & \textbf{0.77}           & 0.33                     & 1.00                    & 0.72                    & \textbf{0.28}            & \textbf{1.00}           & 0.03                    & 0.06                    \\
                                & RC                                & \textbf{1.00}           & 0.36                    & 0.10                     & \textbf{1.00}           & 0.50                    & 0.30                     & 0.99                    & 0.61                    & 0.27                     & 0.89                    & 0.03                    & 0.06                    \\
                                & F1-score                          & 1.00                    & 0.34                    & 0.10                     & \textbf{1.00}           & 0.59                    & 0.31                     & 0.99                    & 0.65                    & 0.28                     & 0.93                    & 0.03                    & 0.06                    \\ \hline
\multirow{3}{*}{llama3.3:70b}   & PR                                & \textbf{0.00}           & \textbf{0.77}           & \textbf{0.19}            & 0.78                    & 0.41                    & 0.29                     & 0.67                    & 0.42                    & 0.17                     & \textbf{1.00}           & 0.01                    & 0.14                    \\
                                & RC                                & \textbf{0.00}           & 0.61                    & 0.16                     & 0.76                    & 0.41                    & 0.25                     & \textbf{0.65}           & 0.43                    & 0.16                     & \textbf{1.00}           & 0.00                    & 0.11                    \\
                                & F1-score                          & \textbf{0.00}           & 0.66                    & 0.17                     & 0.76                    & 0.27                    & 0.27                     & 0.65                    & 0.42                    & 0.16                     & 1.00                    & 0.00                    & 0.12                    \\ \hline
\end{tabular}
\end{adjustbox}

\label{table:comp_aross_hl}
\end{minipage}
\end{table*}

